Execution time budget assignment for mixed criticality systems

In this paper we propose to quantify execution time variability of programs using statistical dispersion parameters. We show how the execution time variability can be exploited in mixed criticality real-time systems. We propose a heuristic to compute the execution time budget to be allocated to each low criticality real-time task according to its execution time variability. We show using experiments and simulations that the proposed heuristic reduces the probability of exceeding the allocated budget compared to algorithms which do not take into account the execution time variability parameter.

==> ARM.tex <==

We generate a set of execution times by executing $1500$ times $8$ programs  from the  TACLeBench \cite{tacle}  in an Arm Cortex A53 processor (4 cores) using the Zynq UltraScale+ MPSoC ZCU104. 
The programs are executed in core 4 using FreeRTOS and rate monotonic scheduling algorithm we consider deadlines  equal to the periods.

We consider the following configuration: (1) we do not variate the inputs of the programs to avoid the variations due to the different input data (2) caches of core 4 are activated to fully exploit the architecture (3) the cores 1, 2 and 3 have there caches not activated and execute a program \cite{CIG} to generate memory contention. This configuration is not the one leading to the worst-case execution time variability since all the programs have single input and the cache of core 4 is activated and thus less memory contention is exhibited. The obtained budgets assure schedulability in this configuration. To compute budgets valid for another configuration, one should use this other configuration to obtain the execution times.

\begin{table}[]
\begin{tabular}{|m{0.8cm}|m{0.5cm}|m{0.5cm}|m{0.5cm}|m{0.4cm}|m{0.4cm}|m{0.45cm}|m{0.7cm}|p{0.7cm}|}
\hline
    % & $P_1$ & $P_2$     & $P_3$ & $P_4$ & $P_5$          & $P_6$         & $P_7$  & $P_8$   \\ \hline
Prog & bs    & bsort & cnt   & edn   & iSort & qSort & ludcmp & matrix1 \\ \hline
T (ms) & 20    & 215       & 35    & 85    & 225            & 165           & 115    & 25      \\ \hline
    \hline
$\frac{BCET}{WCET}$   & 0.005 &  0.01 & 0.13 & 0.59 & 0.13 & 0.26 & 0.1 & 0.69\\
       \hline
sKw & 4 & 9.9 & -0.5 & 14.3 & 4.5 & -15 & 0.7 & 1.2\\
   \hline
VWCET & 96.3 & 92.5 & 52.6 & 35 & 81.1 & 1.8 & 54.4 & 52.4\\
   \hline
    \end{tabular}
    \caption{Variability}
\label{tab:variability}
\end{table}

In Table \ref{tab:variability} we quantify the variability of each program using the quotient between BCET and WCET, the skewness and VWCET parameters. 
% we quantify the variability of each program using the quotient between the BCET and the WCET, the skeweness and the VWCET parameters. We can see that relying on the quotient value is not enough as it shows that most programs have unpredictable temporal behavior, on the contrary of "sKw" and "VWCET" where we can have an idea on the shape of the execution times. 
We note that the quotient value, is not sufficient as an information on the variability of execution times.  % indicates that most programs have unpredictable temporal behavior, however 
In contrast, the "sKw" and "VWCET" parameters provide insight into the tendency of the execution times, for example "cnt" and "iSort" have the same quotient value but using "sKw" and "VWCET" we conclude that the execution times of the first program are more shifted towards it's WCET.

We test Algorithms 1 in two cases: 
\begin{itemize}
        \item VWCET:  Algorithms 1 with $\forall \tau_i$,  $TV_i=VWCET(C_i)$,
    \item  SKw: Algorithms 1 with $\forall \tau_i$,  $TV_i$ is the skeweness of $C_i$
\end{itemize}

We compare Algorithm 1 to the same algorithms used in the simulation-based evaluation minus the algorithm Deadline as deadlines are equal to periods.


 For each program $i$, $Budget_i=\{WCET_i, b_1, b_2, Median_i\}$ where $b_1$ and $b_2$ are the $80th$ and $60th$ percentiles respectively and $Median_i$ is the median value.
\begin{table}[]
\begin{tabular}{|c|c|c|c|cl|cl|cl|}
\hline
Prog   & Medians & Random & Periods & \multicolumn{2}{c|}{sKw}  & \multicolumn{2}{c|}{VWCET} & \multicolumn{2}{c|}{Opt}  \\ \hline
bs  & 0.92    & 0.92   & 0.92   & \multicolumn{2}{c|}{0.92} & \multicolumn{2}{c|}{0.92}  & \multicolumn{2}{c|}{0.92} \\ \hline
bsort & 0.90    & 0.90   & 0.90   & \multicolumn{2}{c|}{0.90} & \multicolumn{2}{c|}{0.90}  & \multicolumn{2}{c|}{0.90} \\ \hline
cnt  & 1       & 1      & 1      & \multicolumn{2}{c|}{1}    & \multicolumn{2}{c|}{1}     & \multicolumn{2}{c|}{1}    \\ \hline
edn & 0.99    & 0.99   & 0.99   & \multicolumn{2}{c|}{0.99} & \multicolumn{2}{c|}{1}     & \multicolumn{2}{c|}{1}    \\ \hline
iSort  & 0.58    & 0.89   & 1      & \multicolumn{2}{c|}{0.89} & \multicolumn{2}{c|}{1}     & \multicolumn{2}{c|}{1}    \\ \hline
qSort  & 0.91    & 1   & 1   & \multicolumn{2}{c|}{1}    & \multicolumn{2}{c|}{1}     & \multicolumn{2}{c|}{1}    \\ \hline
ludcmp  & 0.75    & 0.91   & 0.91   & \multicolumn{2}{c|}{1}    & \multicolumn{2}{c|}{1}     & \multicolumn{2}{c|}{1}    \\ \hline
matrix1 & 1       & 0.80      & 0.80      & \multicolumn{2}{c|}{1}    & \multicolumn{2}{c|}{1}     & \multicolumn{2}{c|}{1}    \\ \hline
$\Pi$  & 0.34    & 0.55   & 0.61   & \multicolumn{2}{c|}{0.75} & \multicolumn{2}{c|}{0.84}  & \multicolumn{2}{c|}{0.84} \\ \hline
\end{tabular}
\caption{Heuristics Scores}
\label{tab:scores}
\end{table}
Table \ref{tab:scores} depicts the scores obtained by every program using every heuristic. The score $\Pi$ is the score computed using Formula 2.  We can see that VWCET have a similar score as the optimal solution, where only two programs "bs" and "bsort" have a probability of exceeding the assigned budget greater than zero.

%\begin{table}
%\caption{Experiments}
%\begin{tabular}{|l|*8{l|}}
%\hline

 %\multicolumn{2}{|l|}{\diagbox{Programs}{Hueristics} }   & sKw & VWCET & All to median & All cases & Periods &Deadlines &Random\\

%\hline
% \multirow{2}{*}{Prog1} & budget & & & & &  & &\\
% \cline{2-9}
% & score &  & & & &  & &\\
%\hline
% \multirow{3}{*}{Prog2} &  budget & & & & & & & \\
% \cline{2-9}
% & score &  & & & &  & &\\
%\hline
% \multirow{2}{*}{Prog3} &  budget &  & & & &   & &\\

% \cline{2-9}
% & score &  & & & &  & &\\
%\hline
% \multirow{2}{*}{Prog4} &  budget &  & & & &  & & \\
% \cline{2-9}
% & score &  & & & & & & \\
%\hline
% \multirow{2}{*}{Prog5} &  budget &  & & & &   & &\\
% \cline{2-9}
% & score &  & & & &  & &\\
%\hline
% \multirow{2}{*}{Prog6} &  budget &  & & & &  & & \\
%  \cline{2-9}
% & score &  & & & &  & & \\
%\hline
% \multirow{2}{*}{Prog7} &  budget &  & & & &   & &\\
% \cline{2-9}
% & score &  & & & &  & & \\
%\hline
%\end{tabular}
%\label{tab:dispertionparameters}
%\end{table}


==> exp.tex <==


\begin{figure}
    \centering
  \begin{tabular}{lcr}
           \includegraphics[width=40mm]{Figures/Mergesort_algorithm.png}     &     \includegraphics[width=40mm]{Figures/Quicksort_algorithm.png}    \\    \includegraphics[width=40mm]{Figures/Insertsort_algorithm.png}
             & 
        \end{tabular}
  
    \caption{Execution times (cycles) of programs executed in an ARM Cortex 53 (4 cores)}
        \label{fig:variability}
\end{figure}

To motivate our approach, Figure \ref{fig:variability} represents histograms of execution times (in terms of number of cycles) of three sorting programs, merge sort, quick sort and insert sort. These three programs perform the same functionality, sorting, but have different variability in execution times.
Let $Q_{merge}$, $Q_{quick}$ and $Q_{insert}$ be the quotient between the worst-case and the best-case execution time for  merge sort, quick sort and insert sort programs respectively with  $Q_{merge}=39659750/35614456=0.898$, $Q_{quick}= 100916776/99806692=0.989$ and $Q_{insert}=19873148/15640168=0.787$. We can see that the more the quotient is small the larger are the execution times. This confirms the fact that reducing the variations in executions time is not always beneficial.

One more point, is that the shape of the histograms of the execution times provides us with more information than the quotient between the worst-case and the best-case execution time (WCET and BCET). Indeed the execution times are left-biased, centered, or right-biased for the same inputs and in the same configuration of the processor i.e. the caches are disabled and one core executes the sorting program and  all other cores execute the same program. This difference is largely due to the number of memory accesses as observed during some experiments made on an Arm Cortex A53 processor and using the provided performance evaluation counters. The execution times of the sorting algorithms were measured in a bare-metal environment using the Zynq UltraScale+ MPSoC ZCU104 Evaluation Kit to avoid the overhead of an operating system.

Given the shape of execution times, one can decide to choose a sorting algorithm according to the time constraints and processor space that one has. For example, if we have enough space in the processor and the program is critical, we can choose the quick sort algorithm, while if the processor is more constrained in space and the program is less critical we can choose the merge sort algorithm while do not considering the worst execution time to estimate the execution time of the program. 

\begin{table}[]
    \caption{Statistical dispersion parameters of execution times of Figure }\ref{fig:variability} 
    \centering
\begin{tabular}{|c|c|c|c|}
\hline
     & Merge sort & Quick sort & Insert sort \\
     \hline
   sKw & 9,559 & -0,399 & -4,186 \\
   \hline
   VWCET & 7,911 & 0,459  & 4,75 \\
   \hline
\end{tabular}

    \label{tab:dispertionparameters}
\end{table}
In Table \ref{tab:dispertionparameters}, the statistical dispersion parameters are presented. 
As we can see, the $sKw$ value is close to zero for quick sort, negative for insert sort and positive for merge sort confirming the shapes of Figure \ref{fig:variability}.
The $VWCET$ value of merge sort is the larger, then follows the $VWCET$ value of insert sort and the $VWCET$ quick sort is the smallest one. 
